HEGEL: Hypergraph Transformer for Long Document Summarization

Extractive summarization for long documents is challenging due to the extended structured input context. The long-distance sentence dependency hinders cross-sentence relations modeling, the critical step of extractive summarization. This paper proposes HEGEL, a hypergraph neural network for long document summarization by capturing high-order cross-sentence relations. HEGEL updates and learns effective sentence representations with hypergraph transformer layers and fuses different types of sentence dependencies, including latent topics, keywords coreference, and section structure. We validate HEGEL by conducting extensive experiments on two benchmark datasets, and experimental results demonstrate the effectiveness and efficiency of HEGEL.

==> table/attn_dist.tex <==

\begin{table}[htbp]
\centering
\small

\begin{tabular}{c| c c c c}
    \hline Hyperedge Type & \makecell{ avg. \\ Attention}& \makecell{ avg. \\  \# Hyperedge}&  \makecell{ avg. \\  \# degree} \Tstrut\Bstrut\\
    \hline Section & \textbf{0.55} & 6.53 & \textbf{15.09}\\
     Topic & 0.28 & \textbf{8.52} & 6.12\\
     Keyword & 0.17 & 4.00 & 7.47\\
    \hline
\end{tabular}
\caption{Average attention distribution over three types of hyperedges on PubMed dataset.}
\label{tab:attention}
\end{table}

==> table/parameters.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c| c}
    \hline Model & Parameters \Tstrut\Bstrut\\
    \hline {\model} &  16 million \\
    SenCLF \& SenPTR & 4.8 million \\ 
    HETERSUMGRAPH & 32 million \\ %\cite{wang-etal-2020-heterogeneous}
    BERTSUMEXTABS & 160 million \\ %\cite{liu2019text}
    \hline
\end{tabular}
\caption{Parameter comparison between different models}
\label{para}
\end{table}

==> table/reachable.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{c| c c c c c}
    \hline \# Answer Nodes & 1 & 2 & 3 & 4 & 5\Tstrut\Bstrut\\
    \hline ROUGE-1 & 45.91 & 47.32 & 48.26 & 46.76 & 47.76 \\
    ROUGE-2 & 18.28 & 20.63 & 22.62 & 21.49 & 22.83 \\
    ROUGE-L & 40.36 & 41.81 & 43.16 & 41.87 & 42.98 \\
    \hline
\end{tabular}

\caption{ROUGE scores over maximum number of answer nodes that one hyperedge can reach within 2 steps of aggregation \haopeng {change into line chart}}
\label{tab:reach}
\end{table}
